Submodularity in conic quadratic mixed 0-1 optimization

We describe strong convex valid inequalities for conic quadratic mixed 0-1 optimization. These inequalities can be utilized for solving numerous practical nonlinear discrete optimization problems from value-at-risk minimization to queueing system design, from robust interdiction to assortment optimization through appropriate conic quadratic mixed 0-1 relaxations. The inequalities exploit the submodularity of the binary restrictions and are based on the polymatroid inequalities over binaries for the diagonal case. We prove that the convex inequalities completely describe the convex hull of a single conic quadratic constraint as well as the rotated cone constraint over binary variables and unbounded continuous variables. We then generalize and strengthen the inequalities by incorporating additional constraints of the optimization problem. Computational experiments on mean-risk optimization with correlations, assortment optimization, and robust conic quadratic optimization indicate that the new inequalities strengthen the convex relaxations substantially and lead to significant performance improvements.

==> tables/assignment15.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
%\caption{Results for assignment with $n=200$ and $m=0$.}
\caption{Results for assignment problem with $n=15$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card0}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{4}{*}{\textbf{6.7\%
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }-\%}&\multicolumn{4}{c|}{\textbf{initial gap: }25.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }37.5\%}&\multicolumn{4}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&-&- & - & - &37.3 & 190,555 & 136 & 0.0 & 29.7 & 1,460,686 & 920 & 0.0 & - & - & - & -\\
&\textbf{Poly1}&-&- & - & - &37.5 & 178,488 & 134 & 0.0 & 30.1 & 1,338,778 & 920 & 0.0 & - & - & - & -\\
&\textbf{Poly2}& - & - & - & - &52.0&94,054 & 94 & 0.0 &49.1 & 955,001 & 1,007 & 0.0 & - & - & - & -\\


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/assignment20.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
%\caption{Results for assignment with $n=200$ and $m=0$.}
\caption{Results for assignment problem with $n=20$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card0}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{4}{*}{\textbf{5\%
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }13.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }21.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }30.5\%}&\multicolumn{4}{c}{\textbf{initial gap: }43.9\%}\\
&\textbf{None}&41.9&2,598,722 & 3,233 & 0.0 &31.9 & 3,690,696 & 6,082 & 4.6 & 25.2 & 4,392,695 & 7,200 & 10.6 & 18.4 & 4,151,017 & 7,200 & 20.7\\
&\textbf{Poly1}&42.2&2,464,741 & 3,452 & 0.1 &31.7 & 3,562,430 & 6,163 & 5.4 & 25.1 & 4,072,906 & 7,200 & 10.6 & 19.1 & 2,860,817 & 7,200 & 22.3\\
&\textbf{Poly2}&52.5&1,986,779 & 3,009 & 0.0 &48.7 & 2,997,580 & 5,944 & 2.8 & 47.4 & 3,500,758 & 7,200 & 6.2 & 45.4 & 3,869,332 & 7,200 & 12.6\\


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/assignment30.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
%\caption{Results for assignment with $n=200$ and $m=0$.}
\caption{Results for assignment problem with $n=30$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card0}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{4}{*}{\textbf{3.3\%
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }11.2\%}&\multicolumn{4}{c|}{\textbf{initial gap: }17.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }23.7\%}&\multicolumn{4}{c}{\textbf{initial gap: }32.7\%}\\
&\textbf{None}&30.5&2,059,641 & 7,200 & 4.9 &19.9 & 1,780,309 & 7,200 & 10.4 & 12.4 & 1,613,567 & 7,200 & 16.2 & 6.3 & 2,768,372 & 7,200 & 24.6\\
&\textbf{Poly1}&32.2&1,746,591 & 7,200 & 5.0 &21.7 & 1,360,323 & 7,200 & 10.6 & 16.7 & 1,211,436 & 7,200 & 16.4 & 12.1 & 1,131,287 & 7,200 & 24.0\\
&\textbf{Poly2}&51.7&1,132,968 & 7,200 & 2.9 &48.9 & 862,926 & 7,200 & 5.9 & 46.3 & 1,090,698 & 7,200 & 9.0 & 45.0 & 853,095 & 7,200 & 13.6\\


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card0.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
%\caption{Results for problem \eqref{eq:computationalB} with $n=200$ and $m=0$.}
\caption{Results for problem \eqref{eq:computationalB}.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card0}
\SingleSpacedXI
\scalebox{0.70}{
\begin{tabular}{ c c | c c c c c | c c c c c | c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Config}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C} &\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]} & \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{20
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }11.4\%}&\multicolumn{5}{c|}{\textbf{initial gap: }17.4\%}&\multicolumn{5}{c}{\textbf{initial gap: }26.8\%}\\
&\textbf{D}&17.4 & 20,197,635 & 6,723 & 2.8[1] & 0 & 3.4 & 13,779,098 & 7,200 & 6.8[0] & 0 & 2.7 & 9,193,790 & 7,200 & 13.1[0] & 0\\
&\textbf{P}&22.3 & 12,862,126 & 6,650 & 2.7[1] & 85 & 10.8 & 13,104,681 & 7,200  & 6.6[0]& 105 & 7.5 & 3,566,591 & 7,200 & 13.7[0] & 89\\
&\textbf{PS}&38.5 & 12,906,403 & 5,950& 1.7[1] & 73  & 30.2 & 16,935,086 & 7,200 & 5.6[0] & 91 & 28.1 & 5,112,724 & 7,200 & 13.4[0] & 60\\

\midrule
&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }3.3\%}&\multicolumn{5}{c}{\textbf{initial gap: }5.6\%}\\
&\textbf{D}&20.7 & 6,235,270 & 1,674 & 0.1[4] &0 & 9.6 & 13,961,488 & 4,360 & 0.4[3] & 0 & 6.0 & 15,334,782 & 6,738 & 1.8[1] & 0\\
&\textbf{P}&70.5 & 620,389 & 261 & 0.0[5] & 63 & 49.2 & 3,268,824 & 2,122 & 0.2[4] & 105 & 30.0 & 6,110,571 & 6,149 & 1.7[1] & 116\\
&\textbf{PS}&75.0 & 90,179 & 62 & 0.0[5] & 58 & 57.3 & 2,729,459 & 1,557 & 0.2[4] & 84 & 42.6 & 5,222,829 & 5,799 & 1.2[1] & 127\\	

\midrule
&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{60
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{5}{c|}{\textbf{initial gap: }0.8\%}&\multicolumn{5}{c}{\textbf{initial gap: }1.4\%}\\
&\textbf{D}&45.8 & 14,387 & 4 & 0.0[5] &0 & 10.9 & 203,275 & 54 & 0.0[5] & 0 & 8.7 & 3,651,174 & 959 & 0.0[5] & 0\\
&\textbf{P}&100.0 & 0 & 1 & 0.0[5] & 4 & 100.0 & 0 & 2 & 0.0[5] & 7 & 86.3 & 1,122 & 5 & 0.0[5] & 47\\
&\textbf{PS}&100.0 & 0 & 1 & 0.0[5] & 7 & 100.0 & 0 & 2 & 0.0[5] & 10 & 94.8 & 262 & 6 & 0.0[5] & 30\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card0New.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
%\caption{Results for problem \eqref{eq:computationalB} with $n=200$ and $m=0$.}
\caption{Results for problem \eqref{eq:computationalB}.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card0}
\SingleSpacedXI
\scalebox{0.70}{
\begin{tabular}{ c c | c c c c c | c c c c c | c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Config}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C} &\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]} & \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{30
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }4.4\%}&\multicolumn{5}{c|}{\textbf{initial gap: }7.2\%}&\multicolumn{5}{c}{\textbf{initial gap: }11.9\%}\\
&\textbf{D}&23.7 & 7,150,715 & 2,528 & 0.3[4] & 0 & 7.2 & 13,632,197 & 6,120 & 1.8[1] & 0 & 4.0 & 16,867,459 & 7,200 & 5.0[0] & 0\\
&\textbf{P}&36.6 & 3,754,826 & 2,073 & 0.4[4] & 65 & 23.7 & 9,573,199 & 5,945  & 1.8[1]& 101 & 14.7 & 10,899,169 & 7,200 & 5.7[0] & 140\\
&\textbf{PS}&48.9 & 2,614,446 & 1,510& 0.2[4] & 73  & 39.8 & 9,235,158 & 5,797 & 1.0[1] & 99 & 31.6 & 13,328,370 & 7,200 & 4.1[0] & 93\\

\midrule
&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }3.3\%}&\multicolumn{5}{c}{\textbf{initial gap: }5.6\%}\\
&\textbf{D}&20.7 & 6,235,270 & 1,674 & 0.1[4] &0 & 9.6 & 13,961,488 & 4,360 & 0.4[3] & 0 & 6.0 & 15,334,782 & 6,738 & 1.8[1] & 0\\
&\textbf{P}&70.5 & 620,389 & 261 & 0.0[5] & 63 & 49.2 & 3,268,824 & 2,122 & 0.2[4] & 105 & 30.0 & 6,110,571 & 6,149 & 1.7[1] & 116\\
&\textbf{PS}&75.0 & 90,179 & 62 & 0.0[5] & 58 & 57.3 & 2,729,459 & 1,557 & 0.2[4] & 84 & 42.6 & 5,222,829 & 5,799 & 1.2[1] & 127\\	

\midrule
&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{50
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.0\%}&\multicolumn{5}{c|}{\textbf{initial gap: }1.6\%}&\multicolumn{5}{c}{\textbf{initial gap: }2.8\%}\\
&\textbf{D}&8.9 & 270,852 & 72 & 0.0[5] &0 & 8.0 & 3,882,494 & 1,045 & 0.0[5] & 0 & 7.9 & 14,835,539 & 4,600 & 0.3[3] & 0\\
&\textbf{P}&93.3 & 249 & 2 & 0.0[5] & 24 & 81.3 & 316,625 & 221 & 0.0[5] & 66 & 57.3 & 4,695,268 & 3,480 & 0.2[3] & 138\\
&\textbf{PS}&93.3 & 98 & 2 & 0.0[5] & 18 & 84.4 & 198,616 & 92 & 0.0[5] & 48 & 64.3 & 983,894 & 1,537 & 0.2[4] & 117\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card100.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} with $n=100$ and $m=100$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card100}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\Omega=1}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=2}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=3}$}&\multicolumn{4}{c }{$\boldsymbol{\Omega=5}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{3}{*}{\textbf{20}}&&\multicolumn{4}{c|}{\textbf{initial gap: }2.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }9.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }22.3\%}&\multicolumn{4}{c}{\textbf{initial gap: }49.3\%}\\
&NONE&10.9&6,507 & 11 & 0.0 &0.0 & 356,548 & 2,403 & 0.0 & 0.0 & 331,661 & 4,182 & 3.1 & 0.0 & 187,566 & 2,637 & 0.7\\
&PU-E  & 18.7 & 7,142 & 9 & 0.0 & 4.6 & 789,132 & 2,905 & 0.5 & 1.9 & 3,402,043 & 4,381 & 2.7 & 2.5 & 146,703 & 3,209 & 2.2  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{50}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.5\%}&\multicolumn{4}{c}{\textbf{initial gap: }20.5\%}\\
&NONE&0.0&53 & 1 & 0.0 &0.0 & 9,383 & 34 & 0.0 & 0.0 & 2,213,370 & 3,465 & 0.3 & 0.0 & 1,378,817 & 7,200 & 10.5\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 73.2 & 3,549 & 67 & 0.0 & 21.9 & 3,706,758 & 4,329 & 0.3 & 4.5 & 741,471 & 7,200 & 12.2  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{80}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{4}{c}{\textbf{initial gap: }4.6\%}\\
&NONE&40.0&35 & 0 & 0.0 &0.0 & 167 & 0 & 0.0 & 0.0 & 8,433 & 129 & 0.0 & 0.0 & 474,880 & 7,200 & 1.9\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 100.0 & 0 & 0 & 0.0 & 92.4 & 86 & 5 & 0.0 & 13.9 & 4,443,350 & 6,796 & 0.9  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{100}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }1.3\%}\\
&NONE&40.0&4 & 0 & 0.0 &0.0 & 58 & 1 & 0.0 & 0.0 & 342 & 6 & 0.0 & 0.0 & 104,693 & 1,401 & 0.0\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 100.0 & 0 & 0 & 0.0 & 86.4 & 20 & 1 & 0.0 & 58.0 & 30,994 & 711 & 0.0  \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card100gradient.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} with gradients, $n=100$ and $m=20$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{5}{*}{\textbf{12
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }18.5\%}&\multicolumn{5}{c|}{\textbf{initial gap: }27.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }44.1\%}\\
&\textbf{None}&21.6 & 486,513 & 363 & 0.0 & 0 & 5.9 & 1,423,492 & 2,387 & 0.2 & 0 & 6.5 & 2,607,095 & 3,804 & 3.2 & 0\\
&\textbf{Poly1}&24.9 & 427,294 & 1,634 & 0.2 & 32 & 19.8 & 2,083,228 & 1,170 & 0.0 & 48 & 6.7 & 2,259,360 & 5,295 & 5.6 & 31\\
&\textbf{Poly2 (B)}&21.0 & 395,119 & 1,186 & 0.0 & 42 & 19.8 & 1,676,430 & 926 & 0.0 & 39 & 8.9 & 2,148,958 & 5,082 & 5.7 & 35\\
&\textbf{Poly2 (B+C)}&29.0 & 423,637 & 1,713 & 1.4 & 134 & 26.2 & 2,683,804 & 1,534 & 0.0 & 65 & 20.7 & 2,972,271 & 5,849 & 10.9 & 167\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{5}{*}{\textbf{18
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }12.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }21.0\%}\\
&\textbf{None}&41.9 & 322,071 & 119 & 0.0 & 0 & 20.8 & 4,045,421 & 1,239 & 0.0 & 0 & 12.1 & 8,980,697 & 5,072 & 1.2 & 0\\
&\textbf{Poly1}&29.7 & 340,492 & 215 & 0.0 & 63 & 18.8 & 3,598,595 & 2,202 & 0.0 & 58 & 10.1 & 6,125,517 & 4,948 & 2.7 & 56\\
&\textbf{Poly2 (B)}&31.9 & 582,119 & 283 & 0.0 & 69 & 16.0 & 3,639,233 & 2,241 & 0.0 & 67 & 10.6 & 5,790,227 & 5,049 & 2.8 & 66\\
&\textbf{Poly2 (B+C)}&32.5 & 239,828 & 180 & 0.0 & 64 & 23.7 & 2,796,604 & 1,707 & 0.0 & 91 & 21.0 & 5,212,827 & 5,020 & 3.1 & 63\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{5}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }3.6\%}&\multicolumn{5}{c|}{\textbf{initial gap: }6.2\%}&\multicolumn{5}{c}{\textbf{initial gap: }10.7\%}\\
&\textbf{None}&56.8 & 23,268 & 8 & 0.0 & 0 & 36.7 & 899,406 & 299 & 0.0 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&53.8 & 20,808 & 11 & 0.0 & 35 & 29.7 & 875,013 & 469 & 0.0 & 82 & - & - & - & - & -\\
&\textbf{Poly2 (B)}&58.8 & 11,643 & 8 & 0.0 & 31 & 28.9 & 2,320,915 & 1,637 & 0.2 & 104 & - & - & - & - & -\\		
&\textbf{Poly2 (B+C)}&57.7 & 8,129 & 13 & 0.0 & 55 & 31.9 & 2,939,848 & 1,806 & 0.2 & 103 & - & - & - & - & -\\


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card100nonlinear.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} with extended formulation, $n=100$ and $m=20$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{12
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }18.5\%}&\multicolumn{5}{c|}{\textbf{initial gap: }27.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }44.1\%}\\
&\textbf{None}&20.3 & 397,816 & 318 & 0.0 & 0 & 11.6 & 1,617,755 & 2,468 & 0.2 & 0 & 4.5 & 2,281,316 & 3,674 & 2.9 & 0\\
&\textbf{Poly1}&20.8 & 540,295 & 275 & 0.0 & 36 & 20.2 & 2,500,122 & 1,246 & 0.0 & 28 & 7.9 & 3,154,258 & 2,881 & 2.7 & 34\\
&\textbf{Poly2}&28.7 & 572,703 & 286 & 0.0 & 33 & 26.1 & 3,207,004 & 1,580 & 0.0 & 35 & 19.5 & 4,164,407 & 3,639 & 2.9 & 41\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{18
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }12.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }21.0\%}\\
&\textbf{None}&39.1 & 223,706 & 87 & 0.0 & 0 & 17.7 & 3,282,604 & 1,315 & 0.0 & 0 & 5.4 & 7,106,310 & 4,836 & 1.4 & 0\\
&\textbf{Poly1}&32.2 & 369,165 & 187 & 0.0 & 44 & 18.9 & 4,048,581 & 2,286 & 0.0 & 47 & 8.0 & 7,150,091 & 4,021 & 1.4 & 38\\
&\textbf{Poly2}&39.2 & 212,285 & 105 & 0.0 & 41 & 20.4 & 2,844,759 & 1,693 & 0.0 & 42 & 24.2 & 8,062,707 & 4,691 & 1.7 & 48\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }3.6\%}&\multicolumn{5}{c|}{\textbf{initial gap: }6.2\%}&\multicolumn{5}{c}{\textbf{initial gap: }10.7\%}\\
&\textbf{None}&44.3 & 26,639 & 8 & 0.0 & 0 & 23.2 & 759,500 & 242 & 0.0 & 0 & 8.7 & 5,359,380 & 2,212 & 0.4 & 0\\
&\textbf{Poly1}&52.1 & 6,129 & 4 & 0.0 & 35 & 28.9 & 1,029,294 & 477 & 0.0 & 41 & 16.9 & 5,053,444 & 4,460 & 0.8 & 45\\
&\textbf{Poly2 }&50.2 & 8,231 & 4 & 0.0 & 38 & 30.8 & 668,883 & 299 & 0.0 & 40 & 22.0 & 6,762,875 & 4,919 & 1.1 & 47\\		


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card100nonlinearUnbounded.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} (unbounded) with extended formulation, $n=100$ and $m=20$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{12
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }17.8\%}&\multicolumn{5}{c|}{\textbf{initial gap: }27.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&9.1 & 255,314 & 84 & 0.0 & 0 & 1.7 & 1,020,747 & 1,650 & 0.0 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&24.7 & 697,234 & 276 & 0.0 & 38 & 27.1 & 2,003,294 & 1,000 & 0.0 & 36 & - & - & - & - & -\\
&\textbf{Poly2}&23.6 & 516,406 & 233 & 0.0 & 39 & 25.0 & 2,737,708 & 1,336 & 0.0 & 33 & - & - & - & - & -\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{18
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&23.3 & 188,778 & 235 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&24.9 & 357,835 & 180 & 0.0 & 34 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2}&22.8 & 369,501 & 155 & 0.0 & 33 & - & - & - & - & - & - & - & - & - & -\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }3.6\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&23.8 & 15,407 & 5 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&42.3 & 10,801 & 6 & 0.0 & 33 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2 }&47.9 & 21,277 & 9 & 0.0 & 31 & - & - & - & - & - & - & - & - & - & -\\		


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card200.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} with $n=200$ and $m=200$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{4}{*}{\textbf{20
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }5.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }8.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }10.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }12.3\%}\\
&\textbf{None}&0.2&118,222 & 4,870 & 0.8 &0.0 & 152,784 & 6,150 & 1.2 & 0.1 & 146,044 & 3,620 & 1.7 & 0.0 & 93,306 & 3,866 & 1.9\\
&\textbf{Poly1}&7.0&713,752 & 5,286 & 0.6 &4.4 & 1,564,590 & 4,776 & 0.9 & 3.3 & 412,284 & 4,245 & 1.4 & 5.3 & 84,735 & 3,842 & 1.7\\
&\textbf{Poly2}&7.8&644,243 & 5,470 & 0.4 &6.6 & 1,663,301 & 4,600 & 0.9 & 7.7 & 636,547 & 4,636 & 1.5 & 11.2 & 63,613 & 3,721 & 1.9\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }1.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }4.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }6.2\%}\\
&\textbf{None}&0.8&78,572 & 2,868 & 0.2 &0.6 & 1,373,294 & 5,710 & 0.5 & 0.3 & 331,777 & 6,004 & 1.7 & 0.0 & 546,551 & 7,200 & 3.1\\
&\textbf{Poly1}&12.5&662,439 & 1,572 & 0.0 &9.6 & 3,067,174 & 6,960 & 0.4 & 4.8 & 1,974,595 & 7,200 & 1.4 & 5.6 & 1,452,010 & 7,200 & 2.6\\
&\textbf{Poly2}&12.9&567,805 & 1,563 & 0.0 &9.0 & 3,434,029 & 6,864 & 0.3 & 6.1 & 2,228,160 & 7,200 & 1.4 & 6.3 & 1,419,926 & 7,200 & 2.6\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{80
}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.2\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{4}{c}{\textbf{initial gap: }1.0\%}\\
&\textbf{None}&9.4&667 & 5 & 0.0 &0.0 & 36,237 & 1,537 & 0.0 & 0.0 & 82,412 & 3,121 & 0.1 & 0.0 & 114,548 & 5,680 & 0.3\\
&\textbf{Poly1}&75.2&21 & 3 & 0.0 &92.1 & 15 & 3 & 0.0 & 70.6 & 2,597 & 15 & 0.0 & 54.0 & 7,792 & 21 & 0.0\\
&\textbf{Poly2}&77.3&23 & 3& 0.0 &93.0 & 26 & 4 & 0.0 & 70.8 & 1,492 & 15 & 0.0 & 52.3 & 4,260 & 46 & 0.0\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card200Final.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB}.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }2.8\%}&\multicolumn{5}{c|}{\textbf{initial gap: }4.2\%}&\multicolumn{5}{c}{\textbf{initial gap: }6.2\%}\\
&\textbf{None}&0.6 & 1,373,294 & 5,710 & 0.5 & 0 & 0.3 & 331,777 & 6,004 & 1.7 & 0 & 0.0 & 546,551 & 7,200 & 3.1 & 0\\
&\textbf{Poly1}&9.6 & 3,067,174 & 6,960 & 0.4 & 45 & 4.8 & 1,974,595 & 7,200 & 1.4 &38 & 5.6 & 1,452,010 & 7,200 & 2.6 & 44\\
&\textbf{Poly2}&9.0 & 3,434,029 & 6,864 & 0.3 & 47 & 6.1 & 2,228,160 & 7,200 & 1.4 & 38 & 6.3 & 1,419,926 & 7,200 & 2.6 & 35\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{80
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{5}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{5}{c}{\textbf{initial gap: }1.0\%}\\
&\textbf{None}&0.0 & 36,237 & 1,537 & 0.0 & 0 & 0.0 & 82,412 & 3,121 & 0.1 & 0 & 0.0 & 114,548 & 5,680 & 0.3 & 0\\
&\textbf{Poly1}&92.1 & 15 & 3 & 0.0 & 17 & 70.6 & 2,597 & 15 & 0.0 & 29 & 54.0 & 7,792 & 21 & 0.0 & 58\\
&\textbf{Poly2}&93.0 & 26 & 4 & 0.0 & 18 &70.8 & 1,492 & 15 & 0.0 &30 & 52.3 & 4,260 & 46 & 0.0 & 63\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card200gradient.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB}.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{5}{*}{\textbf{12
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }18.5\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&0.0 & 222,166 & 1,581 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&8.0 & 234,035 & 3,476 & 0.5 & 25 & - & - & - & - &- & - & - & - & - & -\\
&\textbf{Poly2 (B)}&8.5 & 208,096 & 3,578 & 0.4 & 35 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2 (B+C)}&17.2 & 114,393 & 5,252 & 2.6 & 175 & - & - & - & - & - & - & - & - & - & -\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{5}{*}{\textbf{18
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&0.0 & 190,120 & 1,342 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&18.0 & 173,165 & 2,643 & 0.3 & 29 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2 (B)}&18.7 & 187,419 & 3,253 & 0.5 & 33 &- & - & - & - &- & - & - & - & - & -\\
&\textbf{Poly2 (B+C)}&25.6 & 149,285 & 3,109 & 0.3 & 35 &- & - & - & - &- & - & - & - & - & -\\	

\midrule
&&&&&&&&&&&&&&\\
\multirow{5}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }3.6\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&0.0 & 121,833 & 899 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&38.6 & 141,450 & 2,107 & 0.1 & 29 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2 (B)}&40.6 & 114,741 & 2,071 & 0.2 & 36 &- & - & - & - &- & - & - & - & - & -\\	
&\textbf{Poly2 (B+C)}&43.4 & 89,546 & 1,881 & 0.1 & 41 &- & - & - & - &- & - & - & - & - & -\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card200nonlinear.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB}.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }11.8\%}&\multicolumn{5}{c}{\textbf{initial gap: }17.7\%}\\
&\textbf{None}&13.7 & 10,099,073 & 6,247 & 1.6 & 0 & 2.0 & 4,421,789 & 7,200 & 4.8 & 0 & 1.7 & 2,857,306 & 7,200 & 8.5 & 0\\
&\textbf{Poly1}&13.8 & 9,062,588 & 7,200 & 2.0 & 68 & 9.9 & 5,145,236 & 7,200 & 5.3 &62 & 8.6 & 2,552,574 & 7,200 & 9.0 & 49\\
&\textbf{Poly2}&22.5 & 9,882,517 & 7,200 & 1.6 & 68 & 21.2 & 5,400,458 & 7,200 & 4.4 & 60 & 19.4 & 4,171,920 & 7,200 & 8.4 & 55\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{36
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }2.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }4.8\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&18.8 & 3,778,092 & 1,899 & 0.3 & 0 & 6.8 & 9,258,276 & 5,939 & 1.2 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&31.9 & 1,553,026 & 1,507 & 0.4 & 66 & 20.6 & 5,661,020 & 5,811 & 1.1 & 75 & - & - & - & - & -\\
&\textbf{Poly2}&35.3 & 1,682,350 & 1,543 & 0.3 & 62 &24.7 & 8,187,861 & 5,826 & 1.1 &70 & - & - & - & - & -\\	

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{48
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{5}{c|}{\textbf{initial gap: }2.2\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&30.7 & 258,645 & 146 & 0.0 & 0 & 10.7 & 4,057,982 & 2,363 & 1.1 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&76.2 & 1,540,947 & 1,191 & 0.0 & 47 & 51.7 & 1,322,051 & 1,521 & 0.2 & 76 & - & - & - & - & -\\
&\textbf{Poly2}&76.0 & 1,615,374 & 904 & 0.0 & 46 &52.0 & 1,759,300 & 1,482 & 0.2 &67 & - & - & - & - & -\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card200nonlinearUnbounded.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} (unbounded) with extended formulation, $n=200$ and $m=40$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card200}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{24
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }7.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }11.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&12.3 & 4,704,943 & 6,118 & 2.4 & 0 & 11.9 & 5,063,580 & 7,200 & 4.7 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&13.4 & 5,890,548 & 6,479 & 2.0 & 51 & 8.5 & 6,853,723 & 7,200 & 4.2 & 64 & - & - & - & - & -\\
&\textbf{Poly2}&19.9 & 5,898,778 & 6,459 & 1.9 & 44 & 17.0 & 7,085,544 & 7,200 & 4.0 & 63 & - & - & - & - & -\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{36
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }2.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }4.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&8.1 & 969,225 & 3,209 & 0.5 & 0 & 0.8 & 2,205,427 & 7,200 & 1.7 & 0 & - & - & - & - & -\\
&\textbf{Poly1}&25.5 & 2,185,100 & 1,499 & 0.3 & 59 & 14.9 & 6,616,100 & 5,528 & 1.1 & 75 & - & - & - & - & -\\
&\textbf{Poly2}&29.0 & 2,771,670 & 1,511 & 0.2 & 55 & 15.7 & 6,547,486 & 5,461 & 1.0 & 62 & - & - & - & - & -\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{48
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{5}{c|}{\textbf{initial gap: }-\%}&\multicolumn{5}{c}{\textbf{initial gap: }-\%}\\
&\textbf{None}&12.7 & 1,754,209 & 1,221 & 0.0 & 0 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly1}&69.6 & 393,783 & 223 & 0.0 & 52 & - & - & - & - & - & - & - & - & - & -\\
&\textbf{Poly2 }&72.2 & 664,239 & 348 & 0.0 & 32 & - & - & - & - & - & - & - & - & - & -\\		


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/card50.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalB} with $n=100$ and $m=50$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:card50}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\Omega=1}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=2}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=3}$}&\multicolumn{4}{c }{$\boldsymbol{\Omega=5}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{3}{*}{\textbf{20}}&&\multicolumn{4}{c|}{\textbf{initial gap: }1.5\%}&\multicolumn{4}{c|}{\textbf{initial gap: }10.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }31.6\%}&\multicolumn{4}{c}{\textbf{initial gap: }154.3\%}\\
&NONE&13.0&3,756 & 2 & 0.0 &0.0 & 1,019,265 & 3,320 & 0.5 & 0.0 & 618,340 & 7,200 & 10.9 & 0.0 & 701,502 & 7,200 & 77.9\\
&PU-E  & 43.2 & 2,644 & 2 & 0.0 & 9.6 & 2,215,873 & 3,386 & 1.1 & 3.1 & 2,430,659 & 7,200 & 10.4 & 1.7 & 3,880,013 & 7,200 & 67.8  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{50}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.7\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.8\%}&\multicolumn{4}{c}{\textbf{initial gap: }22.3\%}\\
&NONE&0.0&94 & 0 & 0.0 &0.0 & 3,210 & 19 & 0.0 & 0.0 & 775,455 & 333 & 0.0 & 0.0 & 1,495,891 & 7,200 & 13.1\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 87.3 & 4 & 1 & 0.0 & 30.4 & 392,132 & 268 & 0.0 & 3.9 & 3,370,986 & 7,200 & 12.1  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{80}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }2.5\%}\\
&NONE&20.0&13 & 0 & 0.0 &20.0 & 65 & 0 & 0.0 & 0.0 & 205 & 0 & 0.0 & 0.0 & 237,735 & 2,254 & 0.0\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 100.0 & 0 & 0 & 0.0 & 90.2 & 2 & 0 & 0.0 & 45.6 & 11,773 & 15 & 0.0  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{100}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c}{\textbf{initial gap: }0.4\%}\\
&NONE&100.0&0 & 0 & 0.0 &20.0 & 0 & 0 & 0.0 & 0.0 & 31 & 0 & 0.0 & 0.0 & 520 & 5 & 0.0\\
&PU-E  & 100.0 & 0 & 0 & 0.0 & 100.0 & 0 & 0 & 0.0 & 91.4 & 1 & 0 & 0.0 & 86.4 & 2 & 2 & 0.0  \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal100r10k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=100$ and $k=10$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal100r10k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }4.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }8.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }14.8\%}&\multicolumn{4}{c}{\textbf{initial gap: }27.4\%}\\
&\textbf{None}&11.5&25,717 & 198 & 0.0 &7.3 & 44,635 & 450 & 0.0 & 8.4 & 119,227 & 1,762 & 0.0 & 6.1 & 251,480 & 3,986 & 0.3\\
&\textbf{Poly1}  & 13.1 & 14,657 & 132 & 0.0 & 10.7 & 31,285 & 445 & 0.0 & 8.0 & 144,057 & 2,166 & 0.0 & 7.2 & 277,979 & 5,032 & 0.8  \\
&\textbf{Poly2}  & 15.3 & 11,535 & 105 & 0.0 & 11.9 & 25,919 & 370 & 0.0 & 10.8 & 95,139 & 1,675 & 0.0 & 9.9 & 214,239 & 3,912 & 0.6  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }8.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }16.0\%}&\multicolumn{4}{c|}{\textbf{initial gap: }26.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }48.1\%}\\
&\textbf{None}&19.5&104,864 & 1,923 & 0.3 &12.8 & 279,181 & 4,669 & 2.1 & 6.5 & 443,959 & 7,088 & 6.3 & 3.2 & 333,377 & 7,200 & 19.5\\
&\textbf{Poly1}  & 14.7 & 85,535 & 2,717 & 0.8 & 9.7 & 184,171 & 6,426 & 4.7 & 8.0 & 229,931 & 7,200 & 11.5 & 6.9 & 184,906 & 7,200 & 27.5  \\
&\textbf{Poly2}  & 26.4 & 51,267 & 1,500 & 0.3 & 19.9 & 145,888 & 3,770 & 1.8 & 18.8 & 252,490 & 6,889 & 4.8 & 17.5 & 158,064 & 7,200 & 17.5  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal100r20k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=100$ and $k=20$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal100r20k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }1.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }5.3\%}\\
&\textbf{None}&11.7&10,229 & 139 & 0.0 &3.7 & 44,591 & 609 & 0.0 & 3.6 & 41,797 & 626 & 0.0 & 1.0 & 83,791 & 973 & 0.0\\
&\textbf{Poly1}  & 22.2 & 6,782 & 93 & 0.0 & 22.8 & 14,353 & 206 & 0.0 & 22.1 & 24,833 & 395 & 0.0 & 21.9 & 49,063 & 575 & 0.0  \\
&\textbf{Poly2}  & 20.7 & 6,024 & 67 & 0.0 & 22.5 & 11,238 & 137 & 0.0 & 23.7 & 21,657 & 303 & 0.0 & 23.0 & 36,699 & 520 & 0.0  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }2.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }6.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }10.3\%}\\
&\textbf{None}&7.1&170,568 & 2,013 & 0.0 &6.9 & 192,292 & 3,747 & 0.4 & 2.3 & 305,838 & 6,059 & 1.6 & 0.8 & 348,448 & 7,200 & 3.7\\
&\textbf{Poly1}  & 56.3 & 27,159 & 403 & 0.0 & 44.8 & 87,218 & 2,905 & 0.4 & 36.1 & 136,210 & 4,424 & 0.8 & 29.4 & 224,791 & 6,118 & 2.4  \\
&\textbf{Poly2}  & 59.9 & 10,717 & 169 & 0.0 & 49.6 & 105,604 & 2,779 & 0.2 & 41.8 & 134,139 & 3,196 & 0.4 & 35.8 & 140,326 & 4,557 & 1.5  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal100r40k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=100$ and $k=40$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal100r40k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.2\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.7\%}&\multicolumn{4}{c}{\textbf{initial gap: }1.3\%}\\
&\textbf{None}&6.6&4,637 & 46 & 0.0 &4.6 & 8,719 & 142 & 0.0 & 1.1 & 23,239 & 300 & 0.0 & 0.9 & 65,997 & 991 & 0.0\\
&\textbf{Poly1}  & 24.1 & 2,012 & 29 & 0.0 & 20.9 & 5,184 & 58 & 0.0 & 22.8 & 9,133 & 109 & 0.0 & 22.9 & 20,396 & 337 & 0.0  \\
&\textbf{Poly2}  & 24.0 & 1,886 & 27 & 0.0 & 21.0 & 4,035 & 57 & 0.0 & 22.9 & 9,690 & 92 & 0.0 & 22.5 & 16,931 & 252 & 0.0  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&\textbf{None}&10.6&10,707 & 146 & 0.0 &8.2 & 198,061 & 2,422 & 0.0 & 0.0 & 274,664 & 4,054 & 0.1 & - & - & - & -\\
&\textbf{Poly1}  & 64.9 & 935 & 19 & 0.0 & 66.5 & 8,971 & 108 & 0.0 & 66.9 & 12,791 & 127 & 0.0 & - & - & - & -  \\
&\textbf{Poly2}  & 66.5 & 721 & 12 & 0.0 & 67.7 & 4,754 & 53 & 0.0 & 67.5 & 8,175 & 84 & 0.0 & - & - & - & -  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal20r20k.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=100$, $r=20$ and $k=20$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal20r20k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\Omega=1}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=2}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=3}$}&\multicolumn{4}{c }{$\boldsymbol{\Omega=5}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{3}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.3\%}&\multicolumn{4}{c}{\textbf{initial gap: }137.0\%}\\
&NONE&14.9&126 & 1 & 0.0 &25.2 & 271 & 2 & 0.0 & 31.0 & 585 & 2 & 0.0 & 39.2 & 2,071 & 9 & 0.0\\
&PU-E  & 19.0 & 96 & 0 & 0.0 & 40.2 & 151 & 1 & 0.0 & 50.4 & 232 & 1 & 0.0 & 57.1 & 951 & 5 & 0.0  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{0.5}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }5.9\%}&\multicolumn{4}{c}{\textbf{initial gap: }1315.1\%}\\
&NONE&24.4&245 & 1 & 0.0 &37.9 & 689 & 3 & 0.0 & 26.5 & 3,621 & 9 & 0.0 & 40.0 & 103,851 & 344 & 0.0\\
&PU-E  & 41.2 & 118 & 0 & 0.0 & 57.2 & 431 & 1 & 0.0 & 66.9 & 994 & 3 & 0.0 & 55.1 & 130,829 & 167 & 0.0  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }10.8\%}&\multicolumn{4}{c}{\textbf{initial gap: }$\infty$}\\
&NONE&44.7&485 & 2 & 0.0 &24.1 & 10,969 & 22 & 0.0 & 17.1 & 77,891 & 147 & 0.0 & 37.8 & 429,964 & 2,088 & 6.3\\
&PU-E  & 67.5 & 102 & 0 & 0.0 & 68.9 & 1,828 & 4 & 0.0 & 54.6 & 62,745 & 67 & 0.0 & 51.5 & 1,266,691 & 1,841 & 6.4  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }5.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }19.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }$\infty$}\\
&NONE&41.5&1,427 & 3 & 0.0 &9.2 & 156,963 & 365 & 0.0 & 18.0 & 1,318,260 & 4,225 & 0.9 & 26.9 & 963,401 & 4,314 & -\\
&PU-E  & 84.5 & 69 & 1 & 0.0 & 47.9 & 243,364 & 234 & 0.0 & 31.8 & 3,216,740 & 4,776 & 2.0 & 46.1 & 2,400,183 & 4,317 & -  \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal40r10k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=40$ and $k=10$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal40r10k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }2.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }4.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }7.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }14.3\%}\\
&\textbf{None}&15.0&2,459 & 16 & 0.0 &17.4 & 4,597 & 46 & 0.0 & 18.3 & 7,153 & 57 &0.0&18.0 & 16,490 & 169 &0.0\\
&\textbf{Poly1}  & 17.8 & 3,030 & 20 & 0.0 & 18.5 & 3,518 & 43 & 0.0 & 20.5 & 6,648 & 56 & 0.0 & 17.2 & 18,592 & 156 & 0.0  \\
&\textbf{Poly2}  & 17.5 & 2,073 & 17 & 0.0 & 20.6 & 2,884 & 29 & 0.0 & 21.3 & 3,475 & 33 & 0.0 & 20.5 & 12,882 & 92 & 0.0  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }6.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }12.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }20.1\%}&\multicolumn{4}{c}{\textbf{initial gap: }36.1\%}\\
&\textbf{None}&31.5&30,041 & 243 & 0.0 &26.6 & 126,197 & 1,915 & 0.0 & 23.6 & 353,339 & 5,418 & 1.4 & 17.1 & 362,284 & 7,200 & 9.6\\
&\textbf{Poly1}  & 20.3 & 36,868 & 378 & 0.0 & 13.2 & 232,391 & 4,195 & 0.8 & 11.2 & 354,236 & 6,722 & 5.1 & 9.4 & 253,805 & 7,200 & 15.8  \\
&\textbf{Poly2}  & 29.1 & 17,223 & 132 & 0.0 & 24.4 & 132,503 & 1,311 & 0.0 & 20.1 & 333,780 & 4,938 & 1.4 & 23.0 & 290,118 & 7,200 & 8.7  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal40r20k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=40$ and $k=20$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal40r20k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.7\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.9\%}&\multicolumn{4}{c}{\textbf{initial gap: }3.3\%}\\
&\textbf{None}&13.3&1,387 & 9 & 0.0 &14.3 & 3,882 & 31 & 0.0 & 11.6 & 5,829 & 42 & 0.0 & 17.3 & 7,830 & 80 & 0.0\\
&\textbf{Poly1}  & 21.2 & 1,016 & 7 & 0.0 & 26.6 & 2,456 & 19 & 0.0 & 32.7 & 2,940 & 17 & 0.0 & 29.2 & 7,068 & 69 & 0.0  \\
&\textbf{Poly2}  & 22.6 & 841 & 7 & 0.0 & 28.1 & 2,266 & 17 & 0.0 & 33.4 & 2,232 & 16 & 0.0 & 30.6 & 4,846 & 45 & 0.0  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }1.5\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }5.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }9.0\%}\\
&\textbf{None}&33.9&7,290 & 74 & 0.0 &21.6 & 64,283 & 927 & 0.0 & 15.5 & 240,224 & 3,975 & 0.4 & 6.4 & 378,116 & 7,200 & 2.2\\
&\textbf{Poly1}  & 58.8 & 3,680 & 24 & 0.0 & 55.1 & 14,984 & 165 & 0.0 & 44.4 & 189,826 & 3,380 & 0.4 & 35.7 & 477,553 & 7,200 & 1.9  \\
&\textbf{Poly2}  & 60.7 & 1,733 & 16 & 0.0 & 59.1 & 6,233 & 68 & 0.0 & 50.9 & 102,053 & 1,915 & 0.1 & 43.1 & 430,707 & 5,966 & 0.6  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal40r40k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=200$, $r=40$ and $k=40$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal40r40k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.9}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{4}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{4}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule

\multirow{4}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c}{\textbf{initial gap: }0.8\%}\\
&\textbf{None}&14.9&355 & 3 & 0.0 &8.5 & 1,127 & 9 & 0.0 & 12.7 & 1,209 & 8 & 0.0 & 11.8 & 4,896 & 25 & 0.0\\
&\textbf{Poly1}  & 23.2 & 225 & 2 & 0.0 & 26.0 & 639 & 6 & 0.0 & 32.8 & 635 & 6 & 0.0 & 32.1 & 1,778 & 10 & 0.0  \\
&\textbf{Poly2}  & 23.0 & 226 & 2 & 0.0 & 26.5 & 678 & 7 & 0.0 & 33.1 & 557 & 5 & 0.0 & 32.0 & 1,802 & 9 & 0.0  \\

\midrule
&&&&&&\\
\multirow{4}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }1.0\%}&\multicolumn{4}{c}{\textbf{initial gap: }1.6\%}\\
&\textbf{None}&23.9&4,071 & 24 & 0.0 &23.9 & 6,522 & 64 & 0.0 & 24.0 & 31,022 & 414 & 0.0 & 17.6 & 122,568 & 2,907 & 0.2\\
&\textbf{Poly1}  & 67.3 & 363 & 5 & 0.0 & 72.3 & 270 & 9 & 0.0 & 71.0 & 823 & 12 & 0.0 & 73.9 & 4,416 & 37 & 0.0  \\
&\textbf{Poly2}  & 68.6 & 317 & 5 & 0.0 & 74.8 & 192 & 8 & 0.0 & 72.1 & 695 & 11 & 0.0 & 75.1 & 2,543 & 26 & 0.0  \\

\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal50r20k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=100$, $r=50$ and $k=20$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal50r20k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\Omega=1}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=2}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=3}$}&\multicolumn{4}{c }{$\boldsymbol{\Omega=5}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{3}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }8.7\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&18.1&337 & 1 & 0.0 &2.9 & 4,557 & 12 & 0.0 & 0.0 & 9,400 & 29 & 0.0 & - & - & - & -\\
&PU-E  & 24.0 & 224 & 0 & 0.0 & 27.7 & 2,857 & 6 & 0.0 & 33.1 & 3,883 & 12 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{0.5}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }3.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }11.4\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&23.5&338 & 1 & 0.0 &5.6 & 15,119 & 37 & 0.0 & 4.0 & 31,390 & 113 & 0.0 & - & - & - & -\\
&PU-E  & 45.8 & 140 & 1 & 0.0 & 48.2 & 3,259 & 7 & 0.0 & 52.4 & 13,301 & 28 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }4.8\%}&\multicolumn{4}{c|}{\textbf{initial gap: }16.6\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&16.9&682 & 2 & 0.0 &4.8 & 121,893 & 377 & 0.0 & 3.5 & 281,985 & 1,311 & 0.0 & - & - & - & -\\
&PU-E  & 64.8 & 142 & 1 & 0.0 & 62.8 & 22,421 & 53 & 0.0 & 57.8 & 338,408 & 1,122 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.9\%}&\multicolumn{4}{c|}{\textbf{initial gap: }6.7\%}&\multicolumn{4}{c|}{\textbf{initial gap: }24.1\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&20.1&807 & 2 & 0.0 &2.1 & 898,240 & 2,582 & 0.2 & 1.9 & 1,134,870 & 5,290 & 3.4 & - & - & - & -\\
&PU-E  & 80.4 & 110 & 1 & 0.0 & 51.0 & 747,694 & 2,935 & 0.3 & 41.2 & 990,978 & 4,050 & 3.5 & - & - & - & -  \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonal50r50k.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $n=100$, $r=50$ and $k=50$.}
\setlength{\tabcolsep}{2pt}
\begin{center}
\label{tab:nondiagonal50r50k}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c| c c c c| c c c c| c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{\delta}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{4}{c |}{$\boldsymbol{\Omega=1}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=2}$}&\multicolumn{4}{c |}{$\boldsymbol{\Omega=3}$}&\multicolumn{4}{c }{$\boldsymbol{\Omega=5}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}\\
\midrule
\multirow{3}{*}{\textbf{0.2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.8\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&23.2&91 & 1 & 0.0 &9.1 & 671 & 2 & 0.0 & 4.7 & 1,091 & 3 & 0.0 & - & - & - & -\\
&PU-E  & 24.9 & 61 & 0 & 0.0 & 24.5 & 276 & 1 & 0.0 & 35.9 & 492 & 2 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{0.5}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&11.5&178 & 1 & 0.0 &4.2 & 1,655 & 3 & 0.0 & 0.0 & 2,244 & 6 & 0.0 & - & - & - & -\\
&PU-E  & 35.6 & 73 & 0 & 0.0 & 47.7 & 450 & 1 & 0.0 & 50.7 & 476 & 2 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{1}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.1\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&30.0&167 & 1 & 0.0 &0.0 & 2,472 & 4 & 0.0 & 0.0 & 7,224 & 25 & 0.0 & - & - & - & -\\
&PU-E  & 55.1 & 67 & 0 & 0.0 & 62.0 & 195 & 1 & 0.0 & 63.0 & 803 & 3 & 0.0 & - & - & - & -  \\

\midrule
&&&&&&\\
\multirow{3}{*}{\textbf{2}}&&\multicolumn{4}{c|}{\textbf{initial gap: }0.1\%}&\multicolumn{4}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{4}{c|}{\textbf{initial gap: }2.2\%}&\multicolumn{4}{c}{\textbf{initial gap: }-}\\
&NONE&43.9&136 & 1 & 0.0 &12.5 & 8,407 & 10 & 0.0 & 0.0 & 44,110 & 98 & 0.0 & - & - & - & -\\
&PU-E  & 74.9 & 26 & 0 & 0.0 & 78.6 & 130 & 2 & 0.0 & 82.6 & 464 & 4 & 0.0 & - & - & - & -  \\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonalDelta02Final.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $\delta=0.2$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card02delta}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{20
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{5}{c|}{\textbf{initial gap: }1.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }3.3\%}\\
&\textbf{None}&14.3 & 3,882 & 31 & 0.0 & 0 & 11.6 & 5,829 & 42 & 0.0 & 0 & 17.3 & 7,830 & 80 & 0.0 & 0\\
&\textbf{Poly1}&26.6 & 2,456 & 19 & 0.0 & 19 & 32.7 & 2,940 & 17 & 0.0 &17 & 29.2 & 7,068 & 69 & 0.0 & 69\\
&\textbf{Poly2}&28.1 & 2,266 & 17 & 0.0 & 17 & 33.4 & 2,232 & 16 & 0.0 & 16 & 30.6 & 4,846 & 45 & 0.0 & 45\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{30
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.5\%}&\multicolumn{5}{c|}{\textbf{initial gap: }0.9\%}&\multicolumn{5}{c}{\textbf{initial gap: }1.6\%}\\
&\textbf{None}&17.9 & 1,495 & 10 & 0.0 & 0 & 14.8 & 3,915 & 25 & 0.0 & 0 & 13.7 & 6,554 & 59 & 0.0 & 0\\
&\textbf{Poly1}&28.4 & 890 & 6 & 0.0 & 3 & 28.8 & 2,314 & 13 & 0.0 & 4 & 30.0 & 3,454 & 23 & 0.0 & 6\\
&\textbf{Poly2}&27.0 & 819 & 6 & 0.0 & 2 &28.9 & 1,538 & 11 & 0.0 &5 & 30.5 & 2,605 & 18 & 0.0 & 4\\	

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.3\%}&\multicolumn{5}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{5}{c}{\textbf{initial gap: }0.8\%}\\
&\textbf{None}&8.5 & 1,127 & 9 & 0.0 & 0 & 12.7 & 1,209 & 8 & 0.0 & 0 & 11.8 & 4,896 & 25 & 0.0 & 0\\
&\textbf{Poly1}&26.0 & 639 & 6 & 0.0 & 2 & 32.8 & 635 & 6 & 0.0 & 4 & 32.1 & 1,778 & 10 & 0.0 & 5\\
&\textbf{Poly2}&26.5 & 678 & 7 & 0.0 & 2 &33.1 & 557 & 5 & 0.0 &4 & 32.0 & 1,802 & 9 & 0.0 & 5\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonalDelta05Final.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $\delta=0.5$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card05delta}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{20
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.7\%}&\multicolumn{5}{c|}{\textbf{initial gap: }3.0\%}&\multicolumn{5}{c}{\textbf{initial gap: }5.2\%}\\
&\textbf{D}&22.6 & 9,557 & 74 & 0.0[5] & 0 & 21.3 & 33,468 & 242 & 0.0[5] & 0 & 15.2 & 164,568 & 1,845 & 0.0[5] & 0\\
&\textbf{PU}&53.3 & 3,957 & 23 & 0.0[5] & 13 & 53.5 & 13,316 & 86 & 0.0[5] &15 & 52.8 & 80,735 & 730 & 0.0[5] & 21\\
&\textbf{PS}&55.6 & 2,367 & 17 & 0.0[5] & 10 & 55.9 & 5,839 & 40 & 0.0[5] &14 & 55.3 & 23,577 & 269 & 0.0[5] & 22\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{30
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.8\%}&\multicolumn{5}{c|}{\textbf{initial gap: }1.3\%}&\multicolumn{5}{c}{\textbf{initial gap: }2.3\%}\\
&\textbf{D}&15.5 & 7,115 & 57 & 0.0[5] & 0 & 14.9 & 18,901 & 135 & 0.0[5] & 0 & 5.7 & 76,675 & 1,005 & 0.0[5] & 0\\
&\textbf{PU}&53.3 & 1,656 & 11 & 0.0[5] & 7 & 53.1 & 2,800 & 20 & 0.0[5] & 10 & 61.1 & 8,265 & 48 & 0.0[5] & 13\\
&\textbf{PS}&52.4 & 1,159 & 9 & 0.0[5] & 4 &54.0 & 2,095 & 15 & 0.0[5] &8 & 62.1 & 5,131 & 30 & 0.0[5] & 9\\	

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.4\%}&\multicolumn{5}{c|}{\textbf{initial gap: }0.7\%}&\multicolumn{5}{c}{\textbf{initial gap: }1.1\%}\\
&\textbf{D}&23.3 & 2,910 & 18 & 0.0[5] & 0 & 20.0 & 4,216 & 30 & 0.0[5] & 0 & 13.5 & 46,030 & 514 & 0.0[5] & 0\\
&\textbf{PU}&48.5 & 611 & 6 & 0.0[5] & 4 & 54.3 & 884 & 7 & 0.0[5] & 7 & 55.9 & 2,493 & 18 & 0.0[5] & 8\\
&\textbf{PS}&50.5 & 577 & 6 & 0.0[5] & 4 &55.5 & 839 & 7 & 0.0[5] &8 & 56.7 & 2,144 & 14 & 0.0[5] & 7\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/nondiagonalDelta10Final.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalC} with $\delta=1.0$.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:card10delta}
\SingleSpacedXI
\scalebox{0.8}{
\begin{tabular}{ c c | c c c c c| c c c c c| c c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{k}$}&\multirow{2}{*}{\textbf{Ineq.}} &\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.95}$}&\multicolumn{5}{c |}{$\boldsymbol{\alpha=0.975}$}&\multicolumn{5}{c }{$\boldsymbol{\alpha=0.99}$}\\
&& \textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C}&\textbf{I} & \textbf{N} & \textbf{T} & \textbf{E[S]}& \textbf{C}\\
\midrule
\multirow{4}{*}{\textbf{20
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }2.9\%}&\multicolumn{5}{c|}{\textbf{initial gap: }5.0\%}&\multicolumn{5}{c}{\textbf{initial gap: }9.0\%}\\
&\textbf{D}&21.6 & 64,283 & 927 & 0.0[5] & 0 & 15.5 & 240,224 & 3,975 & 0.4[3] & 0 & 6.4 & 378,116 & 7,200 & 2.2[0] & 0\\
&\textbf{PU}&55.1 & 14,984 & 165 & 0.0[5] & 39 & 44.4 & 189,826 & 3,390 & 0.4[3] &61 & 35.7 & 477,553 & 7,200 & 1.9[0] & 73\\
&\textbf{PS}&59.1 & 6,233 & 68 & 0.0[0] & 28 & 50.9 & 102,053 & 1,915 & 0.1[4] & 35 & 43.1 & 430,707 & 5,966 & 0.6[2] & 53\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{30
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }1.1\%}&\multicolumn{5}{c|}{\textbf{initial gap: }2.0\%}&\multicolumn{5}{c}{\textbf{initial gap: }3.5\%}\\
&\textbf{D}&17.1 & 32,629 & 316 & 0.0[5] & 0 & 12.5 & 150,756 & 2,046 & 0.1[4] & 0 & 10.5 & 258,866 & 3,679 & 0.5[3] & 0\\
&\textbf{PU}&77.2 & 1,082 & 12 & 0.0[5] & 12 & 72.9 & 12,202 & 107 & 0.0[5] & 24 & 67.8 & 115,507 & 1,510 & 0.1[4] & 46\\
&\textbf{PS}&78.2 & 682 & 10 & 0.0[5] & 11 &75.5 & 4,896 & 39 & 0.0[5] &22 & 70.6 & 59,106 & 511 & 0.0[5] & 33\\

\midrule
&&&&&&&&&&&&&&\\
\multirow{4}{*}{\textbf{40
}}&&\multicolumn{5}{c|}{\textbf{initial gap: }0.6\%}&\multicolumn{5}{c|}{\textbf{initial gap: }1.0\%}&\multicolumn{5}{c}{\textbf{initial gap: }1.6\%}\\
&\textbf{D}&23.9 & 6,522 & 64 & 0.0[5] & 0 & 24.0 & 31,022 & 414 & 0.0[5] & 0 & 17.6 & 122,568 & 2,907 & 0.2[3] & 0\\
&\textbf{PU}&72.3 & 270 & 9 & 0.0[5] & 8 & 71.0 & 823 & 12 & 0.0[5] & 11 & 73.9 & 4,416 & 37 & 0.0[5] & 14\\
&\textbf{PS}&74.8 & 192 & 8 & 0.0[5] & 6 &72.1 & 695 & 11 & 0.0[5] &9 & 75.1 & 2,543 & 26 & 0.0[5] & 11\\	


\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/pOFFn100Bar.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} with $n=100$ and presolve OFF - Barrier.}
\begin{center}
\label{tab:pOFFn100Bar}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{Gap}&\textbf{Cuts} \\
\midrule
\multirow{4}{*}{20}&\multirow{4}{*}{1,554.7\%}&NONE&0.0\% & 81,652 & 586 & 0.0\% & 0 \\
&&PU-G & 90.4\% &65,936 &4,676(3) &22.4\%& 78\\
&&PU-E & 90.6\% & 56,557 & 2,084(1) & 1.1\% & 58\\
&&PB& 99.5\% &316 & 25 &0.0\%& 91\\
\midrule
&&&&&&\\
\multirow{4}{*}{50}&\multirow{4}{*}{724.6\%}&NONE&0.0\% & 302,055 & 3,400 & 0.0\% & 0 \\
&&PU-G & 79.7\% &100,949 &7,200 (5)&101.3\%& 70\\
&&PU-E & 79.9\% & 174,282 & 7,200 (5) & 83.0\% & 55 \\
&&PB& 98.8\% &1,635 & 857 & 0.0\% & 176\\
\midrule
&&&&&&\\
\multirow{4}{*}{100}&\multirow{4}{*}{267.8\%}&NONE&0.0\% & 371,308 & 6,050 (4) & 41.2\% & 0 \\
&&PU-G& 70.2\% &96,364 &7,200 (5) &63.9\%& 55\\
&&PU-E &70.4\% & 164,722 & 7,200 (5) & 61.4\% & 50\\
&&PB& 98.7\% &1,506 & 2,959 (2) & 2.0\% & 301\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/pOFFn100Final.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} - presolve OFF.}
\setlength{\tabcolsep}{3pt}
\begin{center}
\label{tab:pOFFn100}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End Gap}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{[Solved]}&\textbf{Cuts} \\
\midrule
\multirow{3}{*}{20}&\multirow{3}{*}{1,554.7\%}&\textbf{D}&0.0\% & 81,652 & 586 & 0.0\%[5] & 0 \\
&&\textbf{PU} & 90.6\% & 56,557 & 2,084 & 1.1\%[4] & 58\\
&&\textbf{PB}& 99.5\% &316 & 25 &0.0\%[5]& 91 \\
\midrule
&&&&&&\\
\multirow{3}{*}{50}&\multirow{3}{*}{724.6\%}&\textbf{D}&0.0\% & 302,055 & 3,400 & 0.0\%[5] & 0 \\
&&\textbf{PU} & 79.9\% & 174,282 & 7,200 & 83.0\%[0]& 55  \\
&&\textbf{PB}& 98.8\% &1,635 & 857 & 0.0\%[5] & 176 \\
\midrule
&&&&&&\\
\multirow{3}{*}{100}&\multirow{3}{*}{267.8\%}&\textbf{D}&0.0\% & 371,308 & 6,050 & 41.2\%[1] & 0 \\
&&\textbf{PU} &70.4\% & 164,722 & 7,200 & 61.4\%[0] & 50 \\
&&\textbf{PB}& 98.7\% &1,506 & 2,959 & 2.0\%[3] & 301\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/pOFFn80Bar.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} with $n=80$ and presolve OFF - Barrier.}
\begin{center}
\label{tab:pOFFn80Bar}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{Gap}&\textbf{Cuts} \\
\midrule
\multirow{4}{*}{16}&\multirow{4}{*}{1,253.8\%}&NONE&0.0\% & 11,214 & 66 & 0.0\% & 0 \\
&&PU-G & 90.6\% &7,939 &483 &0.0\%& 75\\
&&PU-E & 90.9\% & 5,078 & 142 & 0.0\% & 51\\
&&PB& 99.0\% &473 & 23 &0.0\%& 84\\
\midrule
&&&&&&\\
\multirow{4}{*}{40}&\multirow{4}{*}{513.7\%}&NONE&0.0\% & 24,783 & 209 & 0.0\% & 0 \\
&&PU-G & 80.6\% &79,028 &4,825 (3)&25.2\%& 63\\
&&PU-E &80.8\% & 142,148 & 3,965 (2) & 12.1\% & 49\\
&&PB& 98.4\% &245 & 58 & 0.0\% & 134\\
\midrule
&&&&&&\\
\multirow{4}{*}{80}&\multirow{4}{*}{267.3\%}&NONE&0.0\% & 94,932 & 1,134 & 0.0\% & 0 \\
&&PU-G& 69.8\% &113,505 &7,200 (5) &51.6\%& 56\\
&&PU-E& 69.9\% & 229,174 & 7,200 (5) & 42.4\% & 48\\
&&PB& 98.6\% &646 & 278 & 0.0\% & 173\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}


==> tables/pOFFn80OA.tex <==
{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} with $n=80$ and presolve OFF - OA.}
\begin{center}
\label{tab:pOFFn80OA}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{Gap}&\textbf{Cuts} \\
\midrule
\multirow{4}{*}{16}&\multirow{4}{*}{1,253.8\%}&NONE&0.0\% & 190,489 & 7,200 (5)& 1253.8\% & 0 \\
&&PU-G & 54.1\% &86,210 &2,861 (2) &516.6\%& 80\\
&&PU-E & - & - & - & - & -\\
&&PB& 59.8\% &83,260 & 2,867 (2) &519.2\%& 47\\
\midrule
&&&&&&\\
\multirow{4}{*}{40}&\multirow{4}{*}{513.7\%}&NONE&0.0\% & 121,285 & 7,200 (5)& 514.1\% & 0 \\
&&PU-G & 16.4\% &102,673 &5,776 (4)&365.5\%& 68\\
&&PU-E & - & - & - & - & -\\
&&PB& 39.7\% & 59,186 & 4,498 (3)& 334.6\% & 53\\
\midrule
&&&&&&\\
\multirow{4}{*}{80}&\multirow{4}{*}{267.3\%}&NONE&0.0\% & 76,634 & 7,200 (5)& 277.0\% & 0 \\
&&PU-G& 0.0\% &70,995 &7,200 (5) &277.0\%& 4\\
&&PU-E& - & - & - & - & -\\
&&PB& - & - & - & - & -\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/pONn100Bar.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} with $n=100$ and presolve ON.}
\begin{center}
\label{tab:pONn100OA}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{Gap}&\textbf{Cuts} \\
\midrule
\multirow{2}{*}{20}&\multirow{2}{*}{1,554.7\%}&NONE&0.0\% & 283,747 &420 & 0.0\% & 0 \\
&&PU-E & 90.4\% & 19,976 & 628 & 0.0\% & 72\\
\midrule
&&&&&&\\
\multirow{2}{*}{50}&\multirow{2}{*}{724.6\%}&NONE&0.0\% & 1,887,926 & 2,223 & 0.0\% & 0 \\
&&PU-E & 79.4\% & 1,206,283 & 5,770 (4) & 65.4\% & 71 \\
\midrule
&&&&&&\\
\multirow{2}{*}{100}&\multirow{2}{*}{267.8\%}&NONE&0.0\% & 982,945 & 5,343 (3) & 16.1\% & 0 \\
&&PU-E &70.1\% & 615,494 & 7,200 (5) & 54.6\% & 47\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}

==> tables/pONn80OA.tex <==

{
%\SingleSpacedXI
\renewcommand\arraystretch{0.75}
\begin{table}[h!]
\caption{Results for problem \eqref{eq:computationalA} with $n=80$ and presolve ON.}
\begin{center}
\label{tab:pONn80OA}
\SingleSpacedXI
\scalebox{1.0}{
\begin{tabular}{ c c| c |c  c c c c} 
\hline \hline
\multirow{2}{*}{$\boldsymbol{m}$}&\textbf{Initial} &\multirow{2}{*}{\textbf{Config}} &\textbf{Root}&\multirow{2}{*}{\textbf{Nodes}}&\multirow{2}{*}{\textbf{Time}}&\textbf{End}&\textbf{Number}\\
&\textbf{Gap}&&\textbf{Improv.} &&&\textbf{Gap}&\textbf{Cuts} \\
\midrule
\multirow{2}{*}{16}&\multirow{2}{*}{1,253.8\%}&NONE&0.0\% & 16,837 & 25 & 0.0\% & 0 \\
&&PU-E & 90.8\% & 1,748 & 28 & 0.0\% & 57\\
\midrule
&&&&&&\\
\multirow{2}{*}{40}&\multirow{2}{*}{513.7\%}&NONE&0.0\% & 67,685 & 84 & 0.0\% & 0 \\
&&PU-E & 80.3\% & 106,717 & 1,510 (1) & 8.2\% & 74 \\
\midrule
&&&&&&\\
\multirow{2}{*}{80}&\multirow{2}{*}{267.3\%}&NONE&0.0\% & 94,810 & 670 & 0.0\% & 0 \\
&&PU-E &69.7\% & 390,656 & 7,200 (5) & 41.2\% & 35\\
\hline \hline
\end{tabular}
}
\end{center}
\end{table}
}
